SVG-T2I: Scaling Up Text-to-Image Latent Diffusion Model Without Variational Autoencoder

Visual generation grounded in Visual Foundation Model (VFM) representations offers a highly promising unified pathway for integrating visual understanding, perception, and generation. Despite this potential, training large-scale text-to-image diffusion models entirely within the VFM representation space remains largely unexplored. To bridge this gap, we scale the SVG (Self-supervised representations for Visual Generation) framework, proposing SVG-T2I to support high-quality text-to-image synthesis directly in the VFM feature domain. By leveraging a standard text-to-image diffusion pipeline, SVG-T2I achieves competitive performance, reaching 0.75 on GenEval and 85.78 on DPG-Bench. This performance validates the intrinsic representational power of VFMs for generative tasks. We fully open-source the project, including the autoencoder and generation model, together with their training, inference, evaluation pipelines, and pre-trained weights, to facilitate further research in representation-driven visual generation.

==> table/threein1.tex <==
% \begin{table*}[t]
% \centering
% \caption{\textbf{Performance comparison across different models on GenEval~\citep{ghosh2023genevalobjectfocusedframeworkevaluating}, DPG~\citep{dpgbench}, and T2I-CompBench~\citep{t2icompbench}.} 
% $\downarrow$ or $\uparrow$ indicate lower or higher values are better. 
% \textbf{Bold} indicates the best performance, while \underline{underline} denotes the second-best.}
% \label{tab:geneval_dpg_t2icomp}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\#\textbf{Params}} &
% \multicolumn{4}{c}{\textbf{GenEval} $\uparrow$} &
% \multicolumn{4}{c}{\textbf{DPG} $\uparrow$} &
% \multicolumn{3}{c}{\textbf{T2I-CompBench} $\uparrow$} \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-13}
% & & Two Obj. & Counting & Color Att. & Overall & Entity & Relation & Attribute & Overall & Color & Shape & Texture \\
% \midrule
% \multicolumn{13}{c}{\textit{AutoRegressive Models}} \\
% \midrule
% LlamaGen~\citep{llamagen} & 0.8B & 0.34 & 0.21 & 0.04 & 0.32 & - & - & - & 65.16 & - & - & - \\
% Chameleon~\citep{chameleon} & 7B & - & - & - & 0.39 & - & - & - & - & - & - & - \\
% HART~\citep{hart} & 732M & - & - & - & - & - & - & - & 80.89 & - & - & - \\
% Show-o~\citep{show-o} & 1.3B & 0.52 & 0.49 & 0.28 & 0.53 & - & - & - & 67.48 & - & - & - \\
% Emu3~\citep{emu3} & 8.0B & 0.81 & 0.49 & 0.45 & 0.66 & 87.17 & 90.61 & 86.33 & 81.60 & 0.7544 & 0.5706 & 0.7164 \\
% Infinity~\citep{infinity} & 2B & 0.85 & - & 0.57 & 0.73 & - & 90.76 & - & 83.46 & - & - & - \\
% Janus-Pro-1B~\citep{janus-pro} & 1.5B & 0.82 & 0.51 & 0.56 & 0.73 & 88.63 & 88.98 & 88.17 & 82.63 & - & - & - \\
% Janus-Pro-7B~\citep{janus-pro} & 7B & \textbf{0.89} & 0.59 & 0.66 & 0.80 & 88.90 & 89.32 & 89.40 & 84.19 & - & - & - \\
% \midrule
% \multicolumn{13}{c}{\textit{Diffusion Models}} \\
% \midrule
% LDM~\citep{ldm} & 1.4B & 0.29 & 0.23 & 0.05 & 0.37 & - & - & - & 63.18 & - & - & - \\
% SDv1.5~\citep{ldm} & 0.9B & - & - & - & 0.40 & 74.23 & 73.49 & 75.39 & 74.13 & 0.3730 & 0.3646 & 0.4219 \\
% Lumina-Next~\citep{lumina-next} & 1.7B & 0.49 & 0.38 & 0.15 & 0.46 & 83.78 & 89.78 & 82.67 & 75.66 & 0.5088 & 0.3386 & 0.4239 \\
% SDv2.1~\citep{ldm} & 0.9B & 0.51 & 0.44 & 0.50 & 0.47 & - & - & - & 68.09 & 0.5694 & 0.4495 & 0.4982 \\
% PixArt-$\alpha$~\citep{pixartalpha} & 0.6B & 0.50 & 0.44 & 0.07 & 0.48 & 79.32 & 82.57 & 78.60 & 71.11 & 0.6886 & 0.5582 & 0.7064 \\
% SDXL~\citep{sdxl} & 2.6B & 0.74 & 0.39 & 0.23 & 0.55 & 82.43 & 86.76 & 80.91 & 74.65 & 0.6369 & 0.5408 & 0.5637 \\
% SD3-medium~\citep{sd3} & 2B & 0.74 & 0.63 & 0.36 & 0.62 & 91.01 & 80.70 & 88.83 & 84.08 & - & - & - \\
% JanusFlow~\citep{janus-flow} & 1.3B & 0.59 & 0.45 & 0.42 & 0.63 & 87.31 & 89.79 & 87.39 & 80.09 & - & - & - \\
% Sana-0.6B~\citep{sana} & 0.6B & 0.76 & 0.64 & 0.39 & 0.64 & 89.50 & 90.10 & 89.30 & 83.60 & - & - & - \\
% Sana-1.6B~\citep{sana} & 1.6B & 0.77 & 0.62 & 0.47 & 0.66 & 91.50 & 91.90 & 88.90 & 84.80 & - & - & - \\
% DALL-E3~\citep{dalle3} & - & 0.87 & 0.47 & 0.45 & 0.67 & 89.61 & 90.58 & 88.39 & 83.50 & 0.8110 & 0.6750 & 0.8070 \\
% OmniGen~\citep{omnigen} & 3.8B & 0.86 & 0.64 & 0.55 & 0.70 & - & - & - & - & - & - & - \\
% Sana-1.5~\citep{sana} & 4.8B & 0.85 & 0.77 & 0.54 & 0.72 & - & - & - & 85.00 & - & - & - \\
% Lumina-Image 2.0~\citep{lumina2} & 2.6B & 0.87 & 0.67 & 0.62 & 0.73 & 91.97 & 94.85 & 90.20 & 87.20 & 0.8211 & 0.6028 & 0.7417 \\
% \midrule
% \multicolumn{13}{c}{\textit{Representation Generation}} \\
% \midrule
% \textbf{SVG-T2I} & 2.6B & 0.70 & 0.42 & 0.48 & 0.62 & xxx & xxx & xxx & xxx & xxx & xxx & xxx \\
% \textbf{SVG-T2I*} & 2.6B & 0.89 & 0.41 & 0.56 & 0.72 & xxx & xxx & xxx & xxx & xxx & xxx & xxx \\
% % \textbf{SVG-T2I-R-L} & 2.6B & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

